To understand deep learning we need to understand kernel learning

Generalization performance of classifiers in deep learning has recently become a subject of intense study. Deep models, typically over-parametrized, tend to fit the training data exactly. Despite this "overfitting", they perform well on test data, a phenomenon not yet fully understood. The first point of our paper is that strong performance of overfitted classifiers is not a unique feature of deep learning. Using six real-world and two synthetic datasets, we establish experimentally that kernel machines trained to have zero classification or near zero regression error perform very well on test data, even when the labels are corrupted with a high level of noise. We proceed to give a lower bound on the norm of zero loss solutions for smooth kernels, showing that they increase nearly exponentially with data size. We point out that this is difficult to reconcile with the existing generalization bounds. Moreover, none of the bounds produce non-trivial results for interpolating solutions. Second, we show experimentally that (non-smooth) Laplacian kernels easily fit random labels, a finding that parallels results for ReLU neural networks. In contrast, fitting noisy data requires many more epochs for smooth Gaussian kernels. Similar performance of overfitted Laplacian and Gaussian classifiers on test, suggests that generalization is tied to the properties of the kernel function rather than the optimization process. Certain key phenomena of deep learning are manifested similarly in kernel methods in the modern "overfitted" regime. The combination of the experimental and theoretical results presented in this paper indicates a need for new theoretical ideas for understanding properties of classical kernel methods. We argue that progress on understanding deep learning will be difficult until more tractable "shallow" kernel methods are better understood.

==> expr.tex <==
\subsection{Generalization Performance on Synthetic Dataset}
% To investigate the 
% Consider a simple dataset where
\input{figs/synth_lap_klsr_test}


\input{figs/synth_lap_ep_sgd}

\subsection{Interpolating Cases of Shallow Model}


\subsection{Effective Capacity of Shallow Model}


==> figs/interpolate_lap.tex <==
\begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/interpolate/mnist.png}
    \subcaption{MNIST ($6 \cdot 10^4$ samples)}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/interpolate/timit_50k.png}
    \subcaption{TIMIT ($5 \cdot 10^4$ subsamples)}
  \end{minipage}
    \hfill
  \begin{minipage}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{figs/interpolate/hints_50k.png}
    \subcaption{HINT-S ($5 \cdot 10^4$ subsamples)}
  \end{minipage}
  \caption{Interpolation through SGD training for kernel least squares regression (EigenPro-modified Laplace kernel). Top: classification error. Middle: mean squared error (test and train). Bottom: RKHS norm of the model weight.}
  \label{fig:interpolate}
\end{figure}

==> figs/interpolation.tex <==
\begin{figure}[!ht]
  \centering
  \begin{minipage}[b]{0.55\textwidth}
    \includegraphics[width=\textwidth]{figs/ipt-mnist-lap.png}
    \subcaption{MNIST ($\sigma = 10$), $10$ classes}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4125\textwidth}
    \includegraphics[width=\textwidth]{figs/ipt-timit-lap.png}
    \subcaption{TIMIT ($\sigma = 20$), $144$ classes}
  \end{minipage}
  \caption{Histogram of training loss on data points at each epoch}
  \label{fig:interpolation}
\end{figure}

==> figs/lc_norm.tex <==
\begin{wrapfigure}{r}{0.50\textwidth}
  \centering
  \begin{minipage}[b]{.24\textwidth}
    \includegraphics[width=\textwidth]
    {figs/mnist_orig_random_norm_epro.png}         \vspace{-5mm}
    \subcaption{MNIST}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.24\textwidth}
%     \includegraphics[width=\textwidth]
%     {figs/mnist_orig_random_norm_epro.png}
    \vspace{-5mm}
    \subcaption{TIMIT}
  \end{minipage}
  \caption{RKHS norm of overfitted solution}
  \label{fig:lc-norm}
\end{wrapfigure}

==> figs/lc_sgd.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\vspace{-3mm}
\begin{minipage}[b]{.5\textwidth}
  \begin{minipage}[b]{.48\textwidth}
    \includegraphics[width=\textwidth]{figs/mnist_epoch_ratio_epro.png}
    \vspace{-5mm}
    \subcaption{MNIST}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.48\textwidth}
%     \includegraphics[width=\textwidth]
%     {figs/mnist_orig_random_norm_epro.png}
    \vspace{-5mm}
    \subcaption{TIMIT}
  \end{minipage}
  \vspace{-2mm}
  \caption{Epochs to overfit the random label / epochs to overfit the original label}
  \label{fig:lc-ratio}  
\end{minipage}

\vspace{3mm}
\begin{minipage}[b]{.5\textwidth}
  \begin{minipage}[b]{.48\textwidth}
    \includegraphics[width=\textwidth]
    {figs/mnist_orig_random_norm_epro.png}         \vspace{-5mm}
    \subcaption{MNIST}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.48\textwidth}
%     \includegraphics[width=\textwidth]
%     {figs/mnist_orig_random_norm_epro.png}
    \vspace{-5mm}
    \subcaption{TIMIT}
  \end{minipage}
  \vspace{-2mm}
  \caption{RKHS norm of overfitted solution}
  \label{fig:lc-norm} 
\end{minipage}
\end{wrapfigure}

==> figs/lc_synth_real.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
\centering
\vspace{-5mm}
\begin{minipage}[b]{.6\textwidth}
  \begin{minipage}[b]{.49\textwidth}
    \includegraphics[width=\textwidth]
    {figs/synth_lc/syn_0_10_epoch.png}
    \vspace{-5mm}
    \subcaption{Synthetic 1: separable}
    \label{fig:lc-ratio-nsep}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.49\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lc/syn_0_2_epoch.png}
    \vspace{-5mm}
    \subcaption{Synthetic 2: non-separable}
    \label{fig:lc-ratio-nsep}
  \end{minipage}
  
    \begin{minipage}[b]{.49\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lc/mnist_epoch.png}
    \vspace{-5mm}
    \subcaption{MNIST}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.49\textwidth}
    \includegraphics[width=\textwidth]    {figs/synth_lc/svhn_epoch.png}
    \vspace{-5mm}
    \subcaption{SVHN}
  \end{minipage}
  \vspace{-2mm}
  \caption{Ratio: (epochs to overfit random labels) / (epochs to overfit  original labels)}
  \label{fig:lc-ratio}  
\end{minipage}

% \vspace{3mm}
% \begin{minipage}[b]{.5\textwidth}
%   \begin{minipage}[b]{.48\textwidth}
%     \includegraphics[width=\textwidth]
%  {figs/synth_lc/syn_0_2_norm.png}        \vspace{-5mm}
%     \subcaption{Syn. 1: non-separable}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{.48\textwidth}
%     \includegraphics[width=\textwidth]
%     {figs/synth_lc/syn_0_10_norm.png}
%     \vspace{-5mm}
%     \subcaption{Synthetic 2: separable}
%   \end{minipage}
  
%   \begin{minipage}[b]{.48\textwidth}
%     \includegraphics[width=\textwidth]
%     {figs/synth_lc/mnist_norm.png}         \vspace{-5mm}
%     \subcaption{MNIST}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{.48\textwidth}
%     \includegraphics[width=\textwidth]{figs/synth_lc/svhn_norm.png}
%     \vspace{-5mm}
%     \subcaption{SVHN}
%   \end{minipage}
%   \vspace{-2mm}
%   \caption{Ratio of RKHS norm of the solution overfitting the random label to norm of the solution overfitting the original label}
%   \label{fig:lc-norm} 
% \end{minipage}
\end{wrapfigure}

==> figs/normal_dist.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\begin{minipage}[b]{0.5\textwidth}
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figs/ndist_0_10.png}
    \vspace{-5mm}
    \subcaption{separable $C_0$ and $C_1$ ($m_0 = 0, m_1 = 10$)}
    \label{fig:ndist-s}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth]{figs/ndist_0_2.png}
    \vspace{-5mm}
    \subcaption{non-separable $C_0$ and $C_1$ ($m_0 = 0, m_1 = 2$)}
    \label{fig:ndist-ns}
  \end{minipage}
\end{minipage}
  \vspace{-5mm}
  \caption{Probability density of $x_0$}
  \label{fig:ndist}
\end{wrapfigure}

==> figs/synth_0_10_exact.tex <==
\begin{figure}[!h]
  \centering
\begin{minipage}[b]{0.49\textwidth}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10/mse.png}
  \end{minipage}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10/norm.png}
  \end{minipage}
  
    \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10/p001_mse.png}
  \end{minipage}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10/p001_norm.png}
  \end{minipage}

  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10/p01_mse.png}
  \end{minipage}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10/p01_norm.png}
  \end{minipage}
  \subcaption{$m_0 = 0, m_1 = 10$}
  \label{fig:sythn-exact-0-10}
\end{minipage}
\hfill %%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.49\textwidth}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2/mse.png}
  \end{minipage}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2/norm.png}
  \end{minipage}
  
    \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2/p001_mse.png}
  \end{minipage}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2/p001_norm.png}
  \end{minipage}

  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2/p01_mse.png}
  \end{minipage}
  \begin{minipage}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2/p01_norm.png}
  \end{minipage}
  \subcaption{$m_0 = 0, m_1 = 2$}
  \label{fig:sythn-exact-0-2}
\end{minipage}
  \caption{Comparison of direct solutions for kernel least squares regressions (Laplace, $d = 100$) with different sizes of training sets ($n$)
and noises (top: original, middle: 1\% randomly flipped labels, bottom: 10\% randomly flipped labels)}
  \label{fig:sythn-exact}
\end{figure}

==> figs/synth_0_10_lap_ep_sgd.tex <==
\begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_0_10_lap_ep_sgd_train_mse.png}
    \subcaption{mse (train)}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_0_10_lap_ep_sgd_test_mse.png}
    \subcaption{mse (test)}
  \end{minipage}
    \hfill
  \begin{minipage}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_0_10_lap_ep_sgd_test_ce.png}
    \subcaption{classification error (test)}
  \end{minipage}
  \caption{Comparison of error for KLSR (Laplace) models trained by EigenPro iteration on synthetic datasets ($m_0 = 0, m_1 = 10$ for $n = 10^4$ points) with different dimensions ($d$)}
  \label{fig:sythn-sgd}
\end{figure}

==> figs/synth_exact.tex <==
\begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10.png}
    \subcaption{$m_0 = 0, m_1 = 10$}
    \label{fig:sythn-exact-a}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_10_noise_1.png}
    \subcaption{$m_0 = 0, m_1 = 10$, 1\% noise}
    \label{fig:sythn-exact-b}
  \end{minipage}
    \hfill
  \begin{minipage}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth]{figs/lap_0_2.png}
    \subcaption{$m_0 = 0, m_1 = 2$}
    \label{fig:sythn-exact-c}
  \end{minipage}
  \caption{Comparison of exact solutions for kernel least squares regressions (Laplace, $d = 100$) with different sizes of training sets ($n$)}
  \label{fig:sythn-exact}
\end{figure}

==> figs/synth_lap_ep_sgd.tex <==
\begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lap_ep_sgd_train_mse.png}
    \subcaption{mse (train)}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lap_ep_sgd_test_mse.png}
    \subcaption{mse (test)}
  \end{minipage}
    \hfill
  \begin{minipage}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lap_ep_sgd_test_ce.png}
    \subcaption{classification error (test)}
  \end{minipage}
  \caption{Comparison of error for KLSR (Laplace) models trained by EigenPro iteration on synthetic datasets ($n = 10^5$) with different dimensions ($d$)}
  \label{fig:sythn-sgd}
\end{figure}

==> figs/synth_lap_klsr_test.tex <==
\begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lap_klsr_mse.png}
    \subcaption{Loss of the optimal regressor: $0.114$}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lap_klsr_ce.png}
    \subcaption{Bayesian optimal: $15.87\%$}
  \end{minipage}
  \caption{Comparison of testing error for empirical optimal KLSR (Laplace) models on synthetic datasets with different dimension ($d$) and training data size ($n$)}
  \label{fig:sythn-klsr}
\end{figure}

==> figs/synth_lc.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\vspace{-5mm}
\begin{minipage}[b]{.5\textwidth}
  \begin{minipage}[b]{.48\textwidth}
    \includegraphics[width=\textwidth]{figs/synth_lc/syn_0_2_epoch.png}
    \vspace{-5mm}
    \subcaption{Non-separable synth.}
    \label{fig:lc-ratio-nsep}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.48\textwidth}
    \includegraphics[width=\textwidth]
    {figs/synth_lc/syn_0_10_epoch.png}
    \vspace{-5mm}
    \subcaption{Separable synthetic}
    \label{fig:lc-ratio-nsep}
  \end{minipage}
  \vspace{-2mm}
  \caption{(Epochs to overfit the random label) / (epochs to overfit the original label)}
  \label{fig:lc-ratio}  
\end{minipage}

\vspace{3mm}
\begin{minipage}[b]{.5\textwidth}
  \begin{minipage}[b]{.48\textwidth}
    \includegraphics[width=\textwidth]
 {figs/synth_lc/syn_0_2_norm.png}        \vspace{-5mm}
    \subcaption{Non-separable synth.}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{.48\textwidth}
    \includegraphics[width=\textwidth]
    {figs/synth_lc/syn_0_10_norm.png}
    \vspace{-5mm}
    \subcaption{Separable synthetic}
  \end{minipage}
  \vspace{-2mm}
  \caption{(RKHS norm of the solution overfitting the random label) / (norm of the solution overfitting the original label)}
  \label{fig:lc-norm} 
\end{minipage}
\end{wrapfigure}

==> table1_soumik.tex <==
%%Tables for MNIST dataset.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c|c||c|c||c|c||c|c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{8}{c|}{Size of train data} \\ \cline{2-9} 
 & \multicolumn{2}{c||}{$5 \cdot 10^3$} & \multicolumn{2}{c||}{$1.5 \cdot 10^4$} & \multicolumn{2}{c||}{$3 \cdot 10^4$} & \multicolumn{2}{c||}{$6 \cdot 10^4$} \\ \cline{2-9} 
 & EiPro & SGD & EiPro & SGD & EiPro & SGD & EiPro & SGD \\ \hline

Original & 3 & 39 & 7 & 104 & 12 & 204 & 20 & ? \\ \hline

Random & 50 & 684 & 151 & 2210 & 487 & 4966 & 873 & ? \\ \hline

\end{tabular}
\caption{\label{tab:widgets}Comparison of Number of epochs to overfit for EigenPro(EiPro) and Pegasos(SGD) using Gaussian kernel under different levels of noise in labels, and different training data size. Number of epochs to overfit is defined as the epoch when training classification error is 0 . }
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c|c||c|c||c|c||c|c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{8}{c|}{Size of train data} \\ \cline{2-9} 
 & \multicolumn{2}{c||}{$5 \cdot 10^3$} & \multicolumn{2}{c||}{$1.5 \cdot 10^4$} & \multicolumn{2}{c||}{$3 \cdot 10^4$} & \multicolumn{2}{c||}{$6 \cdot 10^4$} \\ \cline{2-9} 
 & EiPro & SGD & EiPro & SGD & EiPro & SGD & EiPro & SGD \\ \hline

Original & 2 & 75 & 3 & 129 & 4 & 141 & 4 & 151 \\ \hline

Random & 4 & 112 & 4 & 131 & 7 & 181 & 7 & 184 \\ \hline

\end{tabular}
\caption{\label{tab:widgets} Comparison of Number of epochs to overfit for EigenPro(EiPro) and Pegasos(SGD) using Laplace kernel under different levels of noise in labels, and different training data size. Number of epochs to overfit is defined as the epoch when training classification error is 0 .  }
\end{table}



% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c|c||c|c||c|c||c|c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{8}{c|}{Size of train data} \\ \cline{2-9} 
 & \multicolumn{2}{c||}{$5 \cdot 10^3$} & \multicolumn{2}{c||}{$1.5 \cdot 10^4$} & \multicolumn{2}{c||}{$3 \cdot 10^4$} & \multicolumn{2}{c||}{$6 \cdot 10^4$} \\ \cline{2-9} 
 & EiPro & SGD & EiPro & SGD & EiPro & SGD & EiPro & SGD \\ \hline

Original & 31 & 26 & 57 & 52 & 83 & 80 & 120 & ? \\ \hline

Random & 136 & 131 & 319 & 305 & 612 & 542 & 1086 & ? \\ \hline

\end{tabular}
\caption{\label{tab:widgets} Comparison of Weight Norms for EigenPro(EiPro) and Pegasos(SGD) using Gaussian kernel under different levels of noise in labels, and different training data size.  }
\end{table}



% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c|c||c|c||c|c||c|c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{8}{c|}{Size of train data} \\ \cline{2-9} 
 & \multicolumn{2}{c||}{$5 \cdot 10^3$} & \multicolumn{2}{c||}{$1.5 \cdot 10^4$} & \multicolumn{2}{c||}{$3 \cdot 10^4$} & \multicolumn{2}{c||}{$6 \cdot 10^4$} \\ \cline{2-9} 
 & EiPro & SGD & EiPro & SGD & EiPro & SGD & EiPro & SGD \\ \hline

Original & 32 & 29 & 54 & 50 & 75 & 66 & 95 & 86 \\ \hline

Random & 74 & 54 & 130 & 100 & 235 & 172 & 333 & 243 \\ \hline

\end{tabular}
\caption{\label{tab:widgets} Comparison of Weight Norms for EigenPro(EiPro) and Pegasos(SGD) using Laplace kernel under different levels of noise in labels, and different training data size.  }
\end{table}

%%Tables for SVHN dataset.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c||c||c||c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{4}{c|}{Size of train data} \\ \cline{2-5} 
 & \multicolumn{1}{c||}{$5 \cdot 10^3$} & \multicolumn{1}{c||}{$1 \cdot 10^4$} & \multicolumn{1}{c||}{$2 \cdot 10^4$} & \multicolumn{1}{c||}{$5 \cdot 10^4$} \\ \cline{2-5} 
 & EiPro & EiPro & EiPro & EiPro \\ \hline

Original & 4 & 9 & 10 & 70 \\ \hline

Random & 5 & 57 & 391 & 752  \\ \hline

\end{tabular}
\caption{\label{tab:widgets}Number of epochs to overfit for EigenPro(EiPro) using Gaussian kernel under different levels of noise in labels, and different training data size. Number of epochs to overfit is defined as the epoch when training classification error is 0 . }
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c||c||c||c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{4}{c|}{Size of train data} \\ \cline{2-5} 
 & \multicolumn{1}{c||}{$5 \cdot 10^3$} & \multicolumn{1}{c||}{$1 \cdot 10^4$} & \multicolumn{1}{c||}{$2 \cdot 10^4$} & \multicolumn{1}{c||}{$5 \cdot 10^4$} \\ \cline{2-5} 
 & EiPro & EiPro & EiPro & EiPro \\ \hline

Original & 2 & 3 & 3 & 9 \\ \hline

Random & 2 & 8 & 14 & 14  \\ \hline

\end{tabular}
\caption{\label{tab:widgets}Number of epochs to overfit for EigenPro(EiPro) using Laplace kernel under different levels of noise in labels, and different training data size. Number of epochs to overfit is defined as the epoch when training classification error is 0 . }
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c||c||c||c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{4}{c|}{Size of train data} \\ \cline{2-5} 
 & \multicolumn{1}{c||}{$5 \cdot 10^3$} & \multicolumn{1}{c||}{$1 \cdot 10^4$} & \multicolumn{1}{c||}{$2 \cdot 10^4$} & \multicolumn{1}{c||}{$5 \cdot 10^4$} \\ \cline{2-5} 
 & EiPro & EiPro & EiPro & EiPro \\ \hline

Original & 66 & 107 & 152 & 298 \\ \hline

Random & 92 & 175 & 276 & 518  \\ \hline

\end{tabular}
\caption{\label{tab:widgets} Weight Norms for EigenPro(EiPro) using Gaussian kernel under different levels of noise in labels, and different training data size.  }
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\label{my-label}
\begin{tabular}{|c||c||c||c||c||}
\hline
\multirow{3}{*}{Label Noise} & \multicolumn{4}{c|}{Size of train data} \\ \cline{2-5} 
 & \multicolumn{1}{c||}{$5 \cdot 10^3$} & \multicolumn{1}{c||}{$1 \cdot 10^4$} & \multicolumn{1}{c||}{$2 \cdot 10^4$} & \multicolumn{1}{c||}{$5 \cdot 10^4$} \\ \cline{2-5} 
 & EiPro & EiPro & EiPro & EiPro \\ \hline

Original & 51 & 84 & 111 & 221 \\ \hline

Random & 56 & 141 & 217 & 352  \\ \hline

\end{tabular}
\caption{\label{tab:widgets}Weight Norms for EigenPro(EiPro) using Laplace kernel under different levels of noise in labels, and different training data size.  }
\end{table}





==> tbls/epoch_gau.tex <==
\begin{wraptable}{r}{7cm}
\centering
% \vspace{-5mm}
\caption{Epochs to overfit (Gaussian)}
\label{tbl:epoch-ep-gau}
\vspace{-2mm}
\resizebox{7cm}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% Label & Syn. 1 & Syn. 2 & MNIST & SVHN & TIMIT \\ \hline
% Original & 1 & 8 & 20 & 46 & 7 \\ \hline
% Random & 635 & 10 & 873 & 1066 & 22 \\ \hline
% \end{tabular}
\begin{tabular}{|c||c|c|c|}
\hline
Label & MNIST & SVHN & TIMIT \\ \hline
Original & 20 & 46 & 7 \\ \hline
Random & 873 & 1066 & 22 \\ \hline
\end{tabular}
}
\vspace{-5mm}
\end{wraptable}

==> tbls/epoch_lap.tex <==
\begin{wraptable}{r}{7cm}
\centering
% \vspace{-5mm}
\caption{Epochs to overfit (Laplacian)}
\label{tbl:epoch-ep-lap}
\vspace{-2mm}
\resizebox{7cm}{!}{
\begin{tabular}{|c||c|c|c|}
\hline
Label & MNIST & SVHN & TIMIT \\ \hline
Original & 4 & 8 & 3 \\ \hline
Random & 7 & 21 & 4 \\ \hline
\end{tabular}
}
\vspace{-5mm}
\end{wraptable}
